Fairness of Exposure in Light of Incomplete Exposure Estimation

Fairness of exposure is a commonly used notion of fairness for ranking systems. It is based on the idea that all items or item groups should get exposure proportional to the merit of the item or the collective merit of the items in the group. Often, stochastic ranking policies are used to ensure fairness of exposure. Previous work unrealistically assumes that we can reliably estimate the expected exposure for all items in each ranking produced by the stochastic policy. In this work, we discuss how to approach fairness of exposure in cases where the policy contains rankings of which, due to inter-item dependencies, we cannot reliably estimate the exposure distribution. In such cases, we cannot determine whether the policy can be considered fair. Our contributions in this paper are twofold. First, we define a method called FELIX for finding stochastic policies that avoid showing rankings with unknown exposure distribution to the user without having to compromise user utility or item fairness. Second, we extend the study of fairness of exposure to the top-k setting and also assess FELIX in this setting. We find that FELIX can significantly reduce the number of rankings with unknown exposure distribution without a drop in user utility or fairness compared to existing fair ranking methods, both for full-length and top-k rankings. This is an important first step in developing fair ranking methods for cases where we have incomplete knowledge about the user's behaviour.

==> references.tex <==


@inproceedings{biega2018equity,
	author = {Biega, Asia J and Gummadi, Krishna P and Weikum, Gerhard},
	booktitle = {The 41st international acm sigir conference on research \& development in information retrieval},
	pages = {405--414},
	title = {Equity of attention: Amortizing individual fairness in rankings},
	year = {2018}}

@inproceedings{singh2018fairness,
	author = {Singh, Ashudeep and Joachims, Thorsten},
	booktitle = {Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
	pages = {2219--2228},
	title = {Fairness of exposure in rankings},
	year = {2018}}

@article{morik2020controlling,
	author = {Morik, Marco and Singh, Ashudeep and Hong, Jessica and Joachims, Thorsten},
	journal = {arXiv preprint arXiv:2005.14713},
	title = {Controlling Fairness and Bias in Dynamic Learning-to-Rank},
	year = {2020}}

@inproceedings{mehrotra2018towards,
  author={Mehrotra, Rishabh and McInerney, James and Bouchard, Hugues and Lalmas, Mounia and Diaz, Fernando},
  booktitle={Proceedings of the 27th acm international conference on information and knowledge management},
  pages={2243--2251},
  title={Towards a fair marketplace: Counterfactual evaluation of the trade-off between relevance, fairness \& satisfaction in recommendation systems},
  year={2018}
} 

@article{wang2020fairness,
  title={Fairness and Diversity for Rankings in Two-Sided Markets},
  author={Wang, Lequn and Joachims, Thorsten},
  journal={arXiv preprint arXiv:2010.01470},
  year={2020}
}
@article{jarvelin2002cumulated,
  title={Cumulated gain-based evaluation of IR techniques},
  author={J{\"a}rvelin, Kalervo and Kek{\"a}l{\"a}inen, Jaana},
  journal={ACM Transactions on Information Systems (TOIS)},
  volume={20},
  number={4},
  pages={422--446},
  year={2002},
  publisher={ACM New York, NY, USA}
}
@article{friedman1996bias,
  title={Bias in computer systems},
  author={Friedman, Batya and Nissenbaum, Helen},
  journal={ACM Transactions on Information Systems (TOIS)},
  volume={14},
  number={3},
  pages={330--347},
  year={1996},
  publisher={ACM New York, NY, USA}
}
@article{zehlike2021fairness,
  title={Fairness in Ranking: A Survey},
  author={Zehlike, Meike and Yang, Ke and Stoyanovich, Julia},
  journal={arXiv preprint arXiv:2103.14000},
  year={2021}
}
@inproceedings{yang2017measuring,
  title={Measuring fairness in ranked outputs},
  author={Yang, Ke and Stoyanovich, Julia},
  booktitle={Proceedings of the 29th International Conference on Scientific and Statistical Database Management},
  pages={1--6},
  year={2017}
}
@inproceedings{zehlike2017fa,
  title={Fa* ir: A fair top-k ranking algorithm},
  author={Zehlike, Meike and Bonchi, Francesco and Castillo, Carlos and Hajian, Sara and Megahed, Mohamed and Baeza-Yates, Ricardo},
  booktitle={Proceedings of the 2017 ACM on Conference on Information and Knowledge Management},
  pages={1569--1578},
  year={2017}
}
@article{baeza2018bias,
  title={Bias on the web},
  author={Baeza-Yates, Ricardo},
  journal={Communications of the ACM},
  volume={61},
  number={6},
  pages={54--61},
  year={2018},
  publisher={ACM New York, NY, USA}
}
@inproceedings{sapiezynski2019quantifying,
  title={Quantifying the Impact of User Attentionon Fair Group Representation in Ranked Lists},
  author={Sapiezynski, Piotr and Zeng, Wesley and E Robertson, Ronald and Mislove, Alan and Wilson, Christo},
  booktitle={Companion Proceedings of The 2019 World Wide Web Conference},
  pages={553--562},
  year={2019}
}
@article{singh2019policy,
  title={Policy learning for fairness in ranking},
  author={Singh, Ashudeep and Joachims, Thorsten},
  journal={arXiv preprint arXiv:1902.04056},
  year={2019}
}
@inproceedings{asudeh2019designing,
  title={Designing fair ranking schemes},
  author={Asudeh, Abolfazl and Jagadish, HV and Stoyanovich, Julia and Das, Gautam},
  booktitle={Proceedings of the 2019 International Conference on Management of Data},
  pages={1259--1276},
  year={2019}
}
@inproceedings{celis2020interventions,
  title={Interventions for ranking in the presence of implicit bias},
  author={Celis, L Elisa and Mehrotra, Anay and Vishnoi, Nisheeth K},
  booktitle={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
  pages={369--380},
  year={2020}
}
@article{celis2017ranking,
  title={Ranking with fairness constraints},
  author={Celis, L Elisa and Straszak, Damian and Vishnoi, Nisheeth K},
  journal={arXiv preprint arXiv:1704.06840},
  year={2017}
}
@inproceedings{geyik2019fairness,
  title={Fairness-aware ranking in search \& recommendation systems with application to linkedin talent search},
  author={Geyik, Sahin Cem and Ambler, Stuart and Kenthapadi, Krishnaram},
  booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={2221--2231},
  year={2019}
}
@inproceedings{stoyanovich2018online,
  title={Online set selection with fairness and diversity constraints},
  author={Stoyanovich, Julia and Yang, Ke and Jagadish, HV},
  booktitle={Proceedings of the EDBT Conference},
  year={2018}
}
@inproceedings{agarwal2019estimating,
  title={Estimating position bias without intrusive interventions},
  author={Agarwal, Aman and Zaitsev, Ivan and Wang, Xuanhui and Li, Cheng and Najork, Marc and Joachims, Thorsten},
  booktitle={Proceedings of the Twelfth ACM International Conference on Web Search and Data Mining},
  pages={474--482},
  year={2019}
}
@inproceedings{ai2018unbiased,
  title={Unbiased learning to rank with unbiased propensity estimation},
  author={Ai, Qingyao and Bi, Keping and Luo, Cheng and Guo, Jiafeng and Croft, W Bruce},
  booktitle={The 41st International ACM SIGIR Conference on Research \& Development in Information Retrieval},
  pages={385--394},
  year={2018}
}
@inproceedings{fang2019intervention,
  title={Intervention harvesting for context-dependent examination-bias estimation},
  author={Fang, Zhichong and Agarwal, Aman and Joachims, Thorsten},
  booktitle={Proceedings of the 42nd International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={825--834},
  year={2019}
}
@inproceedings{joachims2017unbiased,
  title={Unbiased learning-to-rank with biased feedback},
  author={Joachims, Thorsten and Swaminathan, Adith and Schnabel, Tobias},
  booktitle={Proceedings of the Tenth ACM International Conference on Web Search and Data Mining},
  pages={781--789},
  year={2017}
}
@inproceedings{wang2016learning,
  title={Learning to rank with selection bias in personal search},
  author={Wang, Xuanhui and Bendersky, Michael and Metzler, Donald and Najork, Marc},
  booktitle={Proceedings of the 39th International ACM SIGIR conference on Research and Development in Information Retrieval},
  pages={115--124},
  year={2016}
}
@inproceedings{agarwal2019estimating,
  title={Estimating position bias without intrusive interventions},
  author={Agarwal, Aman and Zaitsev, Ivan and Wang, Xuanhui and Li, Cheng and Najork, Marc and Joachims, Thorsten},
  booktitle={Proceedings of the Twelfth ACM International Conference on Web Search and Data Mining},
  pages={474--482},
  year={2019}
}
@inproceedings{ai2018unbiased,
  title={Unbiased learning to rank with unbiased propensity estimation},
  author={Ai, Qingyao and Bi, Keping and Luo, Cheng and Guo, Jiafeng and Croft, W Bruce},
  booktitle={The 41st International ACM SIGIR Conference on Research \& Development in Information Retrieval},
  pages={385--394},
  year={2018}
}
@inproceedings{fang2019intervention,
  title={Intervention harvesting for context-dependent examination-bias estimation},
  author={Fang, Zhichong and Agarwal, Aman and Joachims, Thorsten},
  booktitle={Proceedings of the 42nd International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={825--834},
  year={2019}
}
@inproceedings{wang2018position,
  title={Position bias estimation for unbiased learning to rank in personal search},
  author={Wang, Xuanhui and Golbandi, Nadav and Bendersky, Michael and Metzler, Donald and Najork, Marc},
  booktitle={Proceedings of the Eleventh ACM International Conference on Web Search and Data Mining},
  pages={610--618},
  year={2018}
}

==> sections/discussion.tex <==
%!TEX root = ../main.tex

%\section{Discussion}
% Summarize findings: -Is the top-k ranking method really necessary? 




==> sections/research_questions.tex <==
\section{Research Questions}
\begin{itemize}
    \item Does \method for top-k rankings provide better and more fair top-k results than using the top-k of previous ranking algorithms?
    \item  Can \method effectively avoid showing rankings with unknown exposure distribution?
    \item Can this be done without a significant drop in user utility or item fairness?
    \item How high of a share of rankings with unknown exposure can our method handle?  % This will probably go more into the analysis section 
\end{itemize}

